Stereotypes in Search Engine Results: Understanding The Role of Local and Global Factors

The internet has been blurring the lines between local and global cultures, affecting in different ways the perception of people about themselves and others. In the global context of the internet, search engine platforms are a key mediator between individuals and information. In this paper, we examine the local and global impact of the internet on the formation of female physical attractiveness stereotypes in search engine results. By investigating datasets of images collected from two major search engines in 42 countries, we identify a significant fraction of replicated images. We find that common images are clustered around countries with the same language. We also show that existence of common images among countries is practically eliminated when the queries are limited to local sites. In summary, we show evidence that results from search engines are biased towards the language used to query the system, which leads to certain attractiveness stereotypes that are often quite different from the majority of the female population of the country.

==> discussion.tex <==
\section{Results}

 H1:  Local queries,  global results 
           
           (Os queries sao locais, mas uma ``significativa’’ parte das imagen sao globais. )

Os queries sao locais, mas uma ``significativa’’ parte das imagens
  sao globais.  
                      - descrever o processo automatico de identificacao das imagens repetidas
                      - analisar a distribuicao dessas imagens por classe de query , feias bonitas, etc
                      - analisar por maquina de busca - ha diferenças significativas?
                      - analisar a relação das imagens repetidas com suas posições no ranking de cada pais
                     - analisar imagens repetidas vcs ranking 


    H2: Ranking of results shows discrimination evidences
          
          (indicacoes de discriminação estão presentes no ranking de resultados dos
        queries. Ranking de resultados em ultima instancia definem a visibilidade de imagens)

Indicacoes de discriminação estão presentes no ranking de resultados dos
        queries. Ranking de resultados em ultima instancia definem a visibilidade de imagens.
 
                      - analisar os rankings das consultas, por país, por classe de query, por maquina de 
                        busca
                      - analisar a influencia de ``age'' nos rankings de resultados
                     - analise da influencia de ``race’  nos rankings.


    H3: Query results do not reflect the local demography


